QiMeng-CPU-v2: Automated Superscalar Processor Design by Learning Data Dependencies

Automated processor design, which can significantly reduce human efforts and accelerate design cycles, has received considerable attention. While recent advancements have automatically designed single-cycle processors that execute one instruction per cycle, their performance cannot compete with modern superscalar processors that execute multiple instructions per cycle. Previous methods fail on superscalar processor design because they cannot address inter-instruction data dependencies, leading to inefficient sequential instruction execution. This paper proposes a novel approach to automatically designing superscalar processors using a hardware-friendly model called the Stateful Binary Speculation Diagram (State-BSD). We observe that processor parallelism can be enhanced through on-the-fly inter-instruction dependent data predictors, reusing the processor's internal states to learn the data dependency. To meet the challenge of both hardware-resource limitation and design functional correctness, State-BSD consists of two components: 1) a lightweight state-selector trained by the simulated annealing method to detect the most reusable processor states and store them in a small buffer; and 2) a highly precise state-speculator trained by the BSD expansion method to predict the inter-instruction dependent data using the selected states. It is the first work to achieve the automated superscalar processor design, i.e. QiMeng-CPU-v2, which improves the performance by about $380\times$ than the state-of-the-art automated design and is comparable to human-designed superscalar processors such as ARM Cortex A53.

==> Tex/8_resubmission.tex <==
\clearpage
\setcounter{section}{-1}
\section{Resubmission Information}

 The paper was submitted to NeurIPS 2024. We appreciated that all four  reviewers commend our solid/adequate implementation and evaluation of the hardware design. After some clarification in the rebuttal, all the reviewers approved the originality of this paper, that our work is a new attempt/creation to explore a machine learning processor design application. We are glad to receive a clear accept rating (7), and an above borderline average rating of 4 reviewers (4.75). 
 
 Some of the reviewers concern that the methodology and implementation details are not clear enough.  Our work, encompassing abroad spectrum of research domains (computer architecture, circuit design, and machine learning), is systematic and comprehensive. Since the original NeurIPS manuscript is single-column, some details and preliminaries are relegated to the Appendix. We believe there were significant factual misunderstandings about our methodology and implementation, for example, one reviewer thinks we implement an SMT solver (which is unrealistic and we do not) in the processor hardware and rejects the paper without any further discussion in the rebuttal. We thank all reviewers' dedication and insightful review, and it is our great pleasure to propose this revised manuscript with clearer method/implementation details.
 
For IJCAI 2025, we reorganize the entire Methodology and Implementation section, focusing more on three concepts: 
\begin{itemize}
    \item Design the superscalar processor with dependent data predictor.

\item Train the predictor with S-BSD.

\item Difference between BSD and S-BSD.
\end{itemize}

Besides, to demonstrate the effectiveness of the methodology, we reorganize the Evaluation section focusing more on the comparison of the S-BSD with state-of-the-art methods, human design, best-in-theory design and the ablation study. There is another advancement of this work, that we are now taping out the designed superscalar processor with 28 nm technology. The taped out processor will be manufactured and back for test in May according to the schedule.

\section{Reviews}

In this section, the blue texts are the quoted reviews, and the main texts are our point-by-point responses.

\subsection{Reviewer 43Fz: 7 (confidence 4)}
%Rui：①需要补充一个实验，和带cache的cpu进行对比，reviewer认为结果可能就没有那么好了（①理论上好，②实验结果也好），②可能需要强调一下我们是在和自动化方法对比，而现有的自动化方法都是没有cache的？
%主要问题是性能怎么样，这个可以补一下实验。结果还不错的样子。
\textbf{Summary:}
\textcolor{blue}{This paper proposes a machine learning approach to automatically design superscalar CPUs by value prediction. The authors first formalize automated superscalar processor design as a time series prediction problem. Then the authors propose Stateful Binary Speculation Diagram to learn the on-the-fly predictor. The generated superscalar CPU is evaluated with real-world benchmarks and achieves superior performance than SOTA methods in automatic processor generation.}

\textbf{Soundness:}\textcolor{blue}{ 3: good}

\textbf{Presentation:} \textcolor{blue}{3: good}

\textbf{Contribution:} \textcolor{blue}{3: good}

\textbf{Strengths:}
\textcolor{blue}{This paper innovatively formulates designing super-scalar CPUs as a time series prediction problem. With this formulation, AI could leverage the huge amount of simulation traces to understand the internal structure of CPUs. While value prediction has not been a mainstream way to design a super-scalar CPU, as evidenced by most commercial super-scalar CPU products relying on manually-designed pipelining and out-of-order execution, it might be a suitable starting point for AI to understand how to build a CPU from scratch.}
 
\textcolor{blue}{The authors validate their proposed design with formal verification and logical synthesis, proving the proposed method is practical. The performance of the design is tested with FPGA. The amount of experiment is adequate for an architecture conference paper.}
 
\textcolor{blue}{The problem formulation is concise and clear for the reviewer to quickly grasp the time series prediction problem. The authors also explain the improvement over the baseline BSD method, as well as the misprediction recovery mechanism. The ablation study result is clear to present the effectiveness of your method.}
 
\textcolor{blue}{SOTA methods, and can correctly run various benchmarks, presenting significant progress in automatic CPU designs. Moreover, the proposed state-selector/speculator exhibits great potential by outperforming human expert designs.}

\textbf{Weakness:} \textcolor{blue}{1. An experiment to compare with baseline CPUs with caches should be added.  If your baseline is stronger, I’m skeptical that the improvement of the proposed method may not be as much as the authors claimed. I know it’s probably not possible to add this experiment during rebuttal, but I would like to hear the defense from authors. Could you roughly estimate how much could S-BSD improve over cached baseline CPUs?}

%段落①理论分析我们比带cache的cpu好，②实验结果我们比带cache的cpu好，③强调一下我们是在和自动化方法对比，而现有的自动化方法都是没有cache的？

%第一段：理论上，计算速度由计算和访存决定。cache只解决了访存的问题，我们一种方法通过state prediction的方法,用小的开销预测可以复用的中间结果。这个中间结果可能在访存过程中，也可能在并行计算过程中，如论文中图1所示；这样既解决计算慢的问题，又解决访存慢的问题。

Response: S-BSD improves the processor's performance more than caching. It predicts the intermediate results that can be reused in both the computational part and the memory part, while caching can only accelerate the memory process. In the paper, We compare the performance with human-designed cached CPUs in Section 5.2. 

Our evaluation focuses on comparing the design performance with the state-of-the-art automated design methods, to show how our method significantly narrows the significant performance gap between design by ML methods and design by human experts. Current automated processor designs with state-of-the-art methods cannot analyze the dependencies in the execution so the design has very limited performance than ours without caching or other throughput optimization techniques.

According to your question, we added another experiment to show our method contributes in both the computational part and memory part. With only an extra human-designed cache, the state-of-the-art automated designed CPU \textit{Enlightenment-1}'s throughput is 3985837 Dhrystone/s. The result shows that the memory part introduces 245.7x improvement and the computational part introduces 1.55x improvement compared to the state-of-the-art automated design methods. Thanks for the insightful question and the analysis will be added in the revision.

\textcolor{blue}{2. In figure 2, the illustration could be improved. For instance, the dots in selector region could be aligned. The sub-figure in speculator region could be enlarged.}
%修改图，放在pdf里，传上去（看一下rebuttal改图的要求

Thanks. It will be revised in the revision.

\textbf{Limitations:}
\textcolor{blue}{Yes, the authors claimed that the proposed method is not as good as human designs.}

\textbf{Flag For Ethics Review:} \textcolor{blue}{No ethics review needed.}

\textbf{Rating:} \textcolor{blue}{7: Accept: Technically solid paper, with high impact on at least one sub-area, or moderate-to-high impact on more than one areas, with good-to-excellent evaluation, resources, reproducibility, and no unaddressed ethical considerations.}

\textbf{Confidence:} \textcolor{blue}{4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.}

\textbf{Code Of Conduct:} \textcolor{blue}{Yes}

\subsection{Reviewer Cdjm: 4 (confidence 4)}
%主要问题：
%1. Motivation: 为啥要用这个做依赖分析问题。它对性能影响大，是目前自动化方法做不好的瓶颈。
%2. 方法：S-BSD 和 BSD 的区别，SAT起什么作用

%Rui：这个reviewer的concern是，我们工作预测的dependency prediction是一个【确定性的】，所以他觉得可能没有【预测】或者【自动化】的必要（直接记忆就好了）？所以我们在答的时候需要针对【确定性】说明一下
%①为什么dependency prediction不是确定性任务，②dedendency prediction对于性能很重要，用自动化的动机，用自动化后的意义和重要性

\textbf{Summary:}
\textcolor{blue}{The paper proposes a ML based hardware predictor for detecting instruction dependencies. This is then used to design a superscalar processor with multiple issue width.}

\textbf{Soundness:} \textcolor{blue}{3: good}

\textbf{Presentation:} \textcolor{blue}{3: good}

\textbf{Contribution:} \textcolor{blue}{2: fair}

\textbf{Strengths:}

\textcolor{blue}{Automated creation of data dependency predictors}

\textcolor{blue}{Lightweight solution suitable for hardware implementation}

\textbf{Weakness:} \textcolor{blue}{1. Unclear motivation of why a ML based solution is needed for a deterministic task such as dependency prediction.}

Response 1: Dependent data prediction is not a deterministic task in modern processors in modern processor designs with speculative execution, and the uncertainty comes from changes in the input data of the program. Some of the data, i.e. the predictable data, can be predicted in advance before the execution, which can break the RAW dependencies. We illustrate an example in Figure 1, showing that these optimizations cannot be applied in deterministic techniques such as renaming or reordering. 

%（第二段，为什么我们能做好dependency prediction但是现有ml方法做不好）
%（现在ml方法做不好这个问题的原因是正确性无法保证。accuracy vs coverage预测执行提高性能的一个前提是减少回退，但是ml方法难以达到足够高的准确性。与人工设计相同，我们将）

Our motivation is to explore efficient dependent data prediction methods automatically, i.e. increase the \textit{coverage} of the predictable data. If more data are predictable, according to Def 2.3, the overall throughput can be increased.
However, dependent data prediction is challenging for machine learning methods. Reinforcement Learning [1], Decision Trees [2], and LLMs [3] are used to design small circuit modules, but cannot design large-scale processors accurately. Although the BSD [4] is proposed for ultra-high accurate design, it cannot use inner state information, and thus only design single-cycle processors with limited performance. We meet this challenge with the state selectors and state speculators. The proposed method correctly designs the superscalar processor for the first time, and it can run the Linux OS.

[1]Rajarshi Roy, Jonathan Raiman, Neel Kant, Ilyas Elkin, Robert Kirby, Michael Siu, Stuart Oberman, Saad Godil, and Bryan Catanzaro. Prefixrl: Optimization of parallel prefix circuits using deep reinforcement learning. In Proceedings of Design Automation Conference 853–858. IEEE, 2021

[2] Pei-Wei Chen, Yu-Ching Huang, Cheng-Lin Lee, and Jie-Hong Roland Jiang. Circuit learning for logic regression on high dimensional boolean space. In Proceedings of Design Automation Conference, pages 1–6. IEEE, 2020

[3] Jason Blocklove, Siddharth Garg, Ramesh Karri, and Hammond Pearce. Chip-chat: Challenges and opportunities in conversational hardware design. arXiv preprint arXiv:2305.13243, 2023

[4] Shuyao Cheng, Pengwei Jin, Qi Guo, Zidong Du, Rui Zhang, Yunhao Tian, Xing Hu, Yongwei Zhao, Yifan Hao, Xiangtao Guan, et al. Automated CPU Design by Learning from Input-Output Examples In Proceedings of the International Joint Conference
on Artificial Intelligence, 2024.

%We introduce a novel ML method in this new application, that significantly outperforms the state-of-the-art automated processor design methods, designing high-quality processors comparable with human designs without human involvement.
%也不叫gap吧，就直接说用自动化的手段实现处理器设计？因为将来还是要目标超过人的
%Dependent data prediction is challenging for machine learning methods including LLMs, NNs, Decision Trees, and BSDs, because these methods cannot guarantee design correctness in such high-dimensional design space. In this way, state-of-the-art ML methods can only design single-cycle processors with very limited performance. We meet this challenge with the state selectors and state speculators. The proposed method correctly designs the superscalar processor for the first time, and it can run the Linux OS.

%\textbf{The motivation of the paper is to automatically create hardware units without manual human design. The unit they have explored is the hazard prediction unit that captures data and other dependencies when executing instructions in parallel. I am not sure of the motivation for automated design of this unit. This is a deterministic unit that can accurately calculate whether there is any hazard (RAW, WAR or WAW) and then rename registers on the fly. The only non-determinism comes from branches, which the paper does not elaborate. Please state the motivation clearly in terms of how this would improve hardware design. Automated design is good, but it is unclear to me what advantages it brings for this unit.}

%（第一段，为什么我们要做这件事）我们做的dependency prediction是什么，其实是不确定的task 
%(在预测执行里面，依赖预测不是确定性的问题(这个不确定性来源于程序输入数据的变化)。在这个领域，如图1所示，在出现RAW数据依赖时，会利用speculation的技术提前获得依赖数据，以此提高并行性。相比于传统的确定性dependency analysis将所有RAW依赖都会认为是真相关，更高的预测覆盖率会提高并行性能。人类专家投入很多精力去研究这个问题，自动化设计问题可以降低人类开销，但是获得和人工设计性能相当的设计对ml方法是challenging的。)

%The reviewer gives an example of a classic dependency analysis method, however, the RAW dependencies cannot be executed in parallel with renaming technologies, but can be executed in parallel with dependent data prediction. As shown in Figure 1, some dependent data can be predicted in advance before the execution, which can break the RAW dependencies in a non-deterministic way. Human experts have worked hard for decades to improve the coverage of the dependent data prediction, i.e. to predict more RAW dependent data on-the-fly, outperforming the conservatively determined strategies such as renaming and reordering.




%Besides, automated processor design is currently a important topic in electronic design automation and computer architecture, because it significantly reduce the design cost with considerable performance. In some scenarios, automated methods even outperforms the best human design including pipeline designs, floorplan designs, etc. However, it is still challenging to design high-performance processors end-to-end with ML methods.
%Our method is a breakthrough comparing with the state-of-the-art automated methods for the processor design, while these methods cannot create inner states for the processor to further improve the performance. This paper focus on this specific spot, proposing S-BSD and significantly narrows the gap between the performance of human design and automated design in an industrial scale processor.


\textcolor{blue}{2. Next PC prediction actually falls under branch prediction. This is a much more prudent target since there does not exist a 100\% accurate branch predictor. If the authors can improve on MKPI then that would be a great contribution. There are neural branch predictors used in practice. For instance, consider the HPCA test of time award winning paper [1]. How would your system fare with such an approach?}
%Rui：①关于PC预测，是否可以提升MKPI，为什么（会，不加预测性能会差）②和[1]对比结果怎么样，是否可以一起用

Response 2: Yes, dependent data prediction can improve the MKPI because it is an orthogonal design space compared with the current deterministic methods. More specifically, for the predictable dependent data, the instructions can be executed in parallel due to perfect prediction; and for the unpredictable dependent data, the prediction is bypassed instructions are executed with the current deterministic methods as it should. Besides, the method in [1] can only be used for branch prediction, and cannot be used to predict dependent data in both the computational and memory parts of the processor. It cannot guarantee 100\% prediction accuracy on the predictable data. 

%第一段：accuracy可以达到100\% ，前提是coverage不是100\%，这是现代预测执行的研究惯例。%没有被预测所以是怎么计算的需要提一下 
In dependent data predictions, the accuracy of the prediction needs to achieve 100\% and S-BSD can guarantee the prediction's correctness. To achieve this goal, the predictor does not predict all the possible data, but only the predictable ones. In this way, the metric \textit{coverage} is commonly used in existing value prediction-based studies(and also in this paper), indicating how much data are predictable. The unpredictable data are difficult to predict but it is irrelevant because they can be executed using the conventional deterministic methods including reordering and renaming.  

We give an example here, showing how the predicting accuracy can achieve 100\%. A branch instruction such as $if (a[31:0] > b[31:0]), pc=1000; else pc=8000$. It is difficult to predict the pc without actually executing the instruction with a 32-bit comparison. But in 25\% of the cases, a[31]=1 and b[31]=0, it is very easy to predict the branch and can be formally checked with an SAT solver. Besides, the SAT solver is not on-the-fly in the processor, but a formal verification period while designing the predictor. When the predictor is $(a[31]==1 \&\& b[31]==0) \rightarrow pc=1000$, it is a formally correct predictor, although the predicted coverage is only 25\%. Our ML method is thus motivated to improve the \textit{coverage} of the predictor.

%第二段：MKPI能不能提升？
%可以提升，图1，引用人工设计的预测执行能比不预测性能好的；我们是第一个将这个问题做自动化的工作，用来减少人类开销的同时不太损失性能。
%In this way, dependent data prediction can improve the MKPI because it is an orthogonal design space compared with the current deterministic methods. More specifically, for the ``covered'' dependent data, the instructions can be executed in parallel due to perfect prediction; and for the ``uncovered'' dependent data, the prediction is bypassed instructions are executed with the current deterministic methods as it should. 

%第三段：和[1]的对比
%首先，[1]中的工作只能解决分支预测的问题，对于寄存器值和存储难以实现预测，原因在于更大的设计空间；其次，相比现有的确定性方法，预测执行是一个正交的、更大的设计空间，我们的方法在cover的部分精度做到尽可能高，在没cover的部分仍可以使用传统方法。
%In this way, our system can work with existing methods including the method in [1], because the design space of the proposed method is expanded orthogonally compared with these methods. If the dependent data can be perfectly predicted, our method finds the design; otherwise, all other existing methods can be used as usual.
%Besides, the method in [1] can only be used for branch prediction, and cannot be used to predict dependent data in both the computational and memory parts of the processor. It cannot guarantee 100\% prediction accuracy on the predictable data. 


%Rui：需要写的细致一点，数学一点，摆点公式啥的吧，另外需要强调state信息是如何注入BSD的（在S-BSD里）
\textcolor{blue}{3. Unclear details of the S-BSD model.I am not completely understanding the details between the difference of BSD and S-BSD. Could you provide a mathematical description? It is unclear how the state information is injected into the BSD design.}


Response 3: In short, BSD is only used for combinational logic design without any state information, while S-BSD is capable of designing sequential architectures with unseen states. 
 
Definition 1 is the definition of how BSD design designs a CPU. In this definition, the BSD uses all the readable registers as input-output examples, and fits the CPU with combinational logic.  In this way, the BSD design has the same states as the original design. It can design an ultra-accurate processor but it cannot improve the processor throughput without any structural optimization.
\begin{definition}[CPU Design with BSDs]\label{def:BSD}
There is an \emph{Oracle} $\phi : \left\{0, 1\right\}^n \mapsto \left\{0, 1\right\}^m$, satisfying IO examples of the CPU. Given at most $N$ input-output probes from the oracle $\left\{\left(\mathbf{x}_1, \phi(\mathbf{x}_1)\right), \left(\mathbf{x}_2, \phi(\mathbf{x}_2)\right),\right.$ $\dots,$ $\left.\left(\mathbf{x}_N, \phi(\mathbf{x}_N)\right)\right\}$, construct a Boolean function $\psi$ to simulate $\phi$, 
such that $\forall \mathbf{x} \in \left\{0, 1\right\}^n$,
$$P(\phi (\mathbf{x}) = \psi (\mathbf{x})) \geq 1-\epsilon ~(\epsilon \rightarrow 0),$$  
where the Boolean function $\psi$ is the generated CPU design with BSD. 
\end{definition}

%这里能不能把S-BSD的过程也公式化写一下，另外最好能和上面的def1对比，突出区别，突出state怎么插进BSD里的
The S-BSD explores the parallelism in the design by reusing the intermediate result with states. 
\begin{definition}[CPU design with S-BSD]\label{def:S-BSD}
There is a single-cycle CPU $\Phi : state,inst \rightarrow state$. Build a superscalar CPU $\Phi_{s}: state, inst^k \rightarrow state$, including a $k$ $\Phi$ as execution units and a scheduler built by S-BSD, such that \forall $\omega:inst_0,inst_1,...,inst_n$, the execution result of the final result $inst_n$ is the same.
\end{definition}
In the state selector, S-BSD inserts a small buffer in the predictor, and select which signals to be stored in the buffer. The key challenge in this step is the gap between the large design space for intermediate results and the physical scale limits of the buffer. S-BSD uses a simulated annealing method to efficiently select the more frequently reused signals to buffer.
In the state speculator, S-BSD uses the BSD to design a combinational logic to control the newly inserted buffer. It uses the conventional BSD learning method along with an SAT solver to ensure the correctness of the prediction. More specifically, for the predictable data, the design accuracy has to be 100\% formally. If there are errors and cannot pass the formal verification, we re-train the predictor iterative with more data, while slightly reducing the coverage of the predictor, until it can pass the formal verification.

%加一段：怎么把state注入进来
%引用在文章里面第几行，然后再讲一遍。Figure 2

\textbf{Question:} \textcolor{blue}{1. How do you use SAT solvers in the processor pipeline for error recovery? Do you embed the complete SAT solver? If not, just calling the SAT solver as an external function may be misleading. Since, SAT solver is part of the design it should be embedded into the processor. If so, how costly is it?}
%Rui：①在我们的方法里，SAT solver是怎么使用的，②为什么不会misleading

Answer 1: No, we do not embed any SAT solver in the hardware, so the cost of the solver is irrelevant to the design quality. The SAT solver is used as a formal verification method to check the correctness of the prediction while designing the processor (including the predictor). It is considered as a design/verification period. If the designed processor cannot pass the formal verification with the solver, it is not an acceptable design and we iteratively design another processor until it finally passes the formal verification. 
%\rui{In this way, we defend that our expression does not mislead to readers.}这句去掉吧
%因为它不是part of the processor,所以不需要embed到处理器里面，就不会有cost的问题。我们没有misleading，这个问题的前提是不存在的
%Rui：上一段开头可能要解释一下，为什么不会misleading

\textcolor{blue}{2. I do not understand the last column of Table 3. Is this the prediction accuracy? It says relative. Relative to what?}

Answer 2: No, it is not the prediction accuracy but the prediction coverage. It is the percentage of the coverage of our method to the coverage of the best human design, showing the efficiency of our ML method without any human involvement. The prediction accuracy is 70.69\% reported in Section 5.1.

\textbf{Limitations:}
\textcolor{blue}{The authors mention the limitations saying that the automated design is still not good as human design.}

\textbf{Flag For Ethics Review:} \textcolor{blue}{No ethics review needed.}

\textbf{Rating:} \textcolor{blue}{4: Borderline reject: Technically solid paper where reasons to reject, e.g., limited evaluation, outweigh reasons to accept, e.g., good evaluation. Please use sparingly.}

\textbf{Confidence:} \textcolor{blue}{4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.}

\textbf{Code Of Conduct:} \textcolor{blue}{Yes}

%Rui:rel是什么意思可能需要解释一下
%rel: 占全部predictable的百分比。
%No, the last column of Table 3 shows the \textit{coverage} of the prediction (which is a typical metric in existing value prediction-based methods),
% 可预测的指令片段相对于总执行指令的比例
%i.e. the percentage of predictable data in all possible data. 
%It is not the predicted accuracy. With the SAT solver, we guarantee the predicting accuracy is 100\% in all the predictable data.


\subsection{Reviewer vBrN: 3 (confidence 4)}

\textbf{Summary:}
\textcolor{blue}{Automated processor design is significant challenge given the large design space exploration. The paper proposes Stateful-Binary Speculation Diagram (S-BSD) to design super scalar processors that support pipeline execution. The proposed method uses a simulated annealing based technique to predict the next states of the supposedly state machine for the order of execution of the instructions while identifying the data dependencies.}

\textbf{Soundness:} \textcolor{blue}{2: fair}

\textbf{Presentation:} \textcolor{blue}{2: fair}

\textbf{Contribution:} \textcolor{blue}{3: good}

\textbf{Strengths:}
\textcolor{blue}{The paper is a nice attempt in designing an automated super scalar processor.}

\textcolor{blue}{The results in comparison with the state-of-the-art sound interesting and meeting Human designed Arm Cortex processors through automated design is commendable.}
%主要问题
%1. 算法体现在哪里？为什么需要ML? 类似审稿人2的motivation
%2. 硬件部分：预测如何影响性能？

%\textbf{Unfortunately, there are few concerns that needs to be clarified.}

\textbf{Weakness:} \textcolor{blue}{1. Before all of the concerns, the paper sounds more focused on the processor design while NeurIPS is ML focused. The discussion of ML algorithm, implementation details, ML problem formulation are too small compared to the hardware side of the discussion.}

%Rui：前面我们的topic啥的应该不用写，reviewer也不关心这个，再多重申一下formulation，为什么这个硬件的问题可以转化成ML的问题（时序预测），如果不想再写一遍论文的内容，可以引用一下，论文中的公式几或者定理几写了formulation，另外为什么我们的这个问题是现有ML方法解决不了的也可以再强调一下（并且引用论文中相关部分）

%第一段：我们要做的是把ML应用到processor design里面% 甚至将来要超过人类的设计
Response 1: Our motivation is to apply the ML methods in the automated processor design task, and design high-quality processors without human involvement. 
We introduce a novel ML method in this new application, that significantly outperforms the state-of-the-art automated processor design methods, and design high-quality processors comparable with manual designs without human involvement. It is a challenging for state-of-the-art machine learning methods. Reinforcement Learning [1], Decision Trees [2], LLMs [3] are used to design small-scale circuit modules, but cannot design large-scale processors accurately. Although the BSD [4] is proposed for ultra-high accurate design, it cannot use inner state information, and thus only design single-cycle processors with limited performance. 

%第二段：我们方法的整个流程都是machine learning，首先将问题形式化为时序预测问题，是一个ml问题；然后我们具体的求解方法，包括模拟退火和BSD都是ml方法，整个过程都是ML的。

To achieve this goal, we propose an end-to-end machine learning methodology. First, we formalize the processor design task into a machine learning problem, i.e. the sequential prediction problem. We solve the problem with typical machine learning methods, i.e. the simulated annealing method and the BSD method for the accuracy challenge. The proposed method correctly designs the superscalar processor for the first time, and it can run the Linux OS.

%The key challenge of this specific ML problem is the high design accuracy, so state-of-the-art methods including \rui{Reinforcement Learning [1], Decision Trees~\cite{chen2020circuit}, LLMs~\cite{blocklove2023chip} } cannot design large-scale processors accurately. Although the BSD is proposed for ultra-high accurate design, it cannot use inner state information, and thus only design single-cycle processors with limited performance. We meet the challenge with a state selector learning to reduce the search space, and a state speculator to predict the specific sequence accurately. 

%第三段：我们还和做相同问题的ml方法进行了对比。他们做不好是因为xxx challenge，我们利用xxx ml方法解决了这个问题，性能提高xxx
We evaluate the proposed method with state-of-the-art machine learning methods. Compared with the state-of-the-art automated processor design methods, our method achieves a significant improvement of $382\times$ with the help of dependent data prediction. The design performance is comparable with ARM Cortex A53 CPUs in the 2010s, while no human efforts are involved in our end-to-end machine learning-based design flow.


[1]Rajarshi Roy, Jonathan Raiman, Neel Kant, Ilyas Elkin, Robert Kirby, Michael Siu, Stuart Oberman, Saad Godil, and Bryan Catanzaro. Prefixrl: Optimization of parallel prefix circuits using deep reinforcement learning. In Proceedings of Design Automation Conference 853–858. IEEE, 2021

[2] Pei-Wei Chen, Yu-Ching Huang, Cheng-Lin Lee, and Jie-Hong Roland Jiang. Circuit learning for logic regression on high dimensional boolean space. In Proceedings of Design Automation Conference, pages 1–6. IEEE, 2020

[3] Jason Blocklove, Siddharth Garg, Ramesh Karri, and Hammond Pearce. Chip-chat: Challenges and opportunities in conversational hardware design. arXiv preprint arXiv:2305.13243, 2023

[4] Shuyao Cheng, Pengwei Jin, Qi Guo, Zidong Du, Rui Zhang, Yunhao Tian, Xing Hu, Yongwei Zhao, Yifan Hao, Xiangtao Guan, et al. Automated CPU Design by Learning from Input-Output Examples In Proceedings of the International Joint Conference
on Artificial Intelligence, 2024.


%Our manuscript is submitted for the application topic in the call-for-paper requirement, i.e. \textit{Applications (e.g., vision, language, speech and audio, Creative AI).} We first formalize the superscalar processor design task as an optimization problem, and thus ML methods can be introduced in this new application.

%Besides, processor design is a significant application in computer science. Automated processor design with ML methods have been developed recently, because it significantly reduce the design cost with considerable performance. However, it is still challenging to design high-performance processors end-to-end with ML methods.

%Our method is a breakthrough comparing with the state-of-the-art automated methods for the processor design, while these methods cannot create inner states for the processor to further improve the performance. This paper focus on this specific spot, proposing S-BSD and significantly narrows the gap between the performance of human design and automated design in an industrial scale processor.

\textcolor{blue}{2. There are a few grammatical errors, for example vallina should be vanilla, etc.}

Response 2: Thanks. They will be revised in the revision.

%Rui：①解释为什么需要predictor，②predictor的正确率是100%，解释覆盖率，并且解释那些没用覆盖的数据不影响最终的指令执行结果（即描述一下predictor如果预测错了会怎么执行的过程）

% 1. 确定是需要on-the-fly。为什么需要“on-the-fly”：因为分支、跳转等，离线的模型无法动态获取硬件中实际执行的指令序列，因此无法解除RAW依赖
% 2. 指令执行序列经过一个在线的判断模块，来打上“可预测”和“不可预测”的标签。对于具有“可预测”标签的指令片段，predictor的预测准确率确实是100%，在线解除RAW依赖，能提升处理器性能。对于不可预测的情况，指令序列正常执行，predictor无需处理。

\textbf{Question:} \textcolor{blue}{1. What is the need for an on-the-fly predictor? Is it because the predictor will be deployed in the real hardware for performing real-time speculation?}

%第一段：为什么需要predictor，（第二个审稿人一样，预测会提高性能，如图1）。是的，这是处理器的一部分，去perform real-time speculation.

Answer 1: Yes, the predictor will be deployed in the real hardware. The on-the-fly predictor is needed in the modern processor design periods to further improve the performance with RAW dependencies.  Offline model (e.g. in the compiler) lacks the execution intermediate result information so that they cannot predict accurate-enough results.
%As shown in Figure 1, some dependent data can be predicted in advance before the execution, which can break the RAW dependencies. Human experts have worked hard for decades to improve the coverage of dependent data prediction, i.e. to predict more RAW dependent data on-the-fly, outperforming the conservatively determined strategies such as renaming and reordering.

%第二段：yes 对可预测的部分我们确实要做到100%，但是覆盖率不会达到100%；这是现代预测执行的研究惯例。如果没有覆盖到，我们就不进行预测执行，用现有的传统处理器分析方法即可，不会损失性能。

\textcolor{blue}{2. If that is the case, shouldn’t this predictor be 100\% accurate? If the predictor is not deployed rather used as a one off model that helps drive the design decision of a generic processor then the speed is not really an issue. In either of the cases accuracy certainly should be perfect.}

Answer 2: Yes, the accuracy of the proposed predictor is perfect, which is guaranteed with formal verification in an SAT solver. In the on-the-fly execution, every instruction is classified as predictable and unpredictable. For the predictable instructions, the predicted accuracy is 100\%; and for the unpredictable instructions, the instructions can be executed using the conventional deterministic methods including reordering and renaming. 

%To achieve this goal, we do not predict all the data, but only part of them. The metric ``coverage'' is commonly used in existing value prediction-based methods (and also in this paper), indicating that how much data can be predicted. The ``covered'' data need to be predicted perfectly, and the proposed S-BSD method with an SAT solver guarantees the design correctness.
%The ``uncover'' data can be difficult to predict but it is irrelevant because these are not predicted at all. These data can be executed using the conventional deterministic methods including reordering and renaming.

\textcolor{blue}{3. will the predictor offer more parallelization possibilities, if so will it be stable and consistent in its predictions? }

Answer 3: Yes, it is a hardware implementation within the processor. The on-the-fly predictor is a sub-module of the processor so that it is hardware-implemented and stable/consistent with all computing workloads. To demonstrate this feature, we run real-world CPU benchmarks, i.e. Dhrystone/Linux OS, on the processor design, which includes all types of workloads.

\textcolor{blue}{4. For example, consider the following case: i) will the runtime be (approximately) same to run the same program with same data when run multiple times? ii) if we run the same program but change the data will it produce the same parallelization strategy or will it suggest a different one?}
%Rui：①预测是否是stable and consistent的，②和人比怎么样

Answer 4:
i) Yes, the runtime is approximately the same in every run, and the Dhrystone benchmark actually includes runs millions of times and outputs the average performance.
ii)Yes, the hardware implemented predictor will produce a stable parallel strategy, although the runtime is slightly different in each run because of the dynamic physical information while execution challenges with different data and different runs. In large-scale programs, the performance difference is not significant, and close to the average performance in multiple runs.

\textcolor{blue}{5. If it suggests an efficient one, that adapts to the data, how does the performance of that fare against that of the ones designed by humans?}

Answer 5: In the evaluation section 5.2, Page 8 Line 275, we compare our design with the human design. Our proposed method gets comparable results as the human design, while reducing all the effort of experienced human designers. 
Comparing with the state-of-the-art, our method significantly narrows the gap between the performance of human design and automated design in an industrial scale processor.In this way, the proposed method significantly narrows the gap between the human design and current ML methods.

\textcolor{blue}{6. Eq. 3 is concerning, it is not clear as to how the $Acc(CPU_{p})$ can be combined with $L_{p}$. How can one interpret the relation between the accuracy of a predictor, the latency and the through per instruction. It is understandable the relation between the TPI and latency but how does accuracy of a predictor help $TPI(CPU_{p})$ estimation/optimization. How is this empirical equation deduced?
Also, this equation looks like a multi-objective optimization function, it is not clear if the whole equation is optimized by simulated annealing or is it just the predictor part that is being optimized?}
%变形一下公式，表示是个单目标优化，acc是和模拟退火要优化的东西相关的

Answer 6: The equation is used as the reward function of the simulated annealing method, formalizing the superscalar processor design task into an optimization problem. 

It is a single-objective optimization, according to definition 2.3, we only optimize the total predicting accuracy Acc(P). In our design, we optimize one object, i.e. the \textit{coverage} of the predictor: for x\% of the data (the predictable data), the predicted accuracy is 100\% perfectly; and for the rest of the data, the predictor is invalid, and stall the execution awaiting the RAW dependent data to be executed.

In this way, the predictable data (the probability is Acc(P)) are predicted to execute in parallel and the latency is $L_p$; Otherwise (the probability is 1-Acc(P)), the predictor is invalid, and the dependent data has to be executed with average latency of TPI(CPU). We calculate the mathematical expectations of the latency, i.e. TPI($CPU_p$) and it is Eq. 3
\begin{equation}
       \mathrm{TPI}(\mathrm{CPU}_p) = L_p \times \mathrm{Acc}(\mathrm{CPU}_p) + \mathrm{TPI}(\mathrm{CPU})\times(1-\mathrm{Acc}(\mathrm{CPU}_p))
\end{equation}



\textcolor{blue}{7. All of sudden we see PC, GPR and MEM, three predictors for each of them. How is the proposed approach cohesively aligning with the three of the hardware components. Are there 3 models or one model that considers everything into play?}

Answer 7: The on-the-fly predictor implements 3 hardware models, and each of the models are used to predict the dependent data for PC/GPR/MEM respectively. As discussed in Section 4, PC/GPR/MEM are the only three elements in the processor with data dependencies.

\textcolor{blue}{8. Finally, what is the impact of Cache/RAM on the latency/throughput prediction in this paper altogether?}

%\rui{This is the main idea of how dependency data prediction optimize the processor performance.}
%这个表述很奇怪，改成 The main idea of this work is predicting dependency data to optimize the processor performance.

Answer 8: The prediction and Cache/RAM are orthogonal methods. Cache/RAM are used to optimize the data access latency (just like manual designs), which can improve the processor throughput at the program level. The prediction reuses the data in the Cache/RAM, bypassing the execution latency in the RAW dependencies, which improve the processor throughput at the instruction level. 

%The latency of getting the data from the buffer (including Cache/RAM) is much quicker than the actual execution. The main idea of this paper is to effectively take advantage of this impact, and design high-quality processors automatically.
﻿
%More specifically, RAW dependencies cannot execute in parallel with conventional dependency analysis. The latency awaiting the dependent data to be executed can be reduced with an on-the-fly predictor, reusing the intermediate results from the buffer. This optimization is called "speculative execution" in the processor design, which can make the processor thus much quicker.
﻿
%For example, as shown in Figure 1. Without a buffer to predict the result of the dependent data r1, the total latency is 2 clock cycles. With the buffer to predict r1, these two instructions can be executed in parallel, and the total latency is 1 clock cycle.

\textbf{Limitations:} \textcolor{blue}{Limitations are not discussed at all.}

Response: We discuss the limitations in Page 9 Line 321. It can also be referred from other reviewer.

\textbf{Flag For Ethics Review:} \textcolor{blue}{No ethics review needed.}

\textbf{Rating:} \textcolor{blue}{3: Reject: For instance, a paper with technical flaws, weak evaluation, inadequate reproducibility and/or incompletely addressed ethical considerations.}

\textbf{Confidence:} \textcolor{blue}{4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.}

\textbf{Code Of Conduct:} \textcolor{blue}{Yes}

\subsection{Reviewer qqkn: 5 (confidence 3)}
%主要问题：
%1. 算法体现在哪里? 同审稿人3问题
%2. 实验结果？ 同审稿人1问题

\textbf{Summary:}
\textcolor{blue}{This paper presents an automated superscalar processor design framework aimed at enhancing the performance of processors created without human intervention. By utilizing an automated value predictor, Stateful Binary Speculation Diagram, the framework effectively addresses data dependencies between instructions, facilitating parallel execution. The proposed architecture efficiently extracts data dependencies from the processor's internal state space. This approach achieves performance improvements of approximately 380x over single-cycle processors designed using current state-of-the-art methods.}

\textbf{Soundness:} \textcolor{blue}{3: good}

\textbf{Presentation:} \textcolor{blue}{3: good}

\textbf{Contribution:} \textcolor{blue}{2: fair}

\textbf{Strengths:}
\textcolor{blue}{The pros of the paper are listed below:}

\textcolor{blue}{Extension of State-of-the-Art Methods: The paper extends the state-of-the-art method of automatic CPU generation, specifically the BSD method, to superscalar CPU architectures, demonstrating a notable application of existing techniques.}

\textcolor{blue}{Functional Demonstration: The automatically generated CPU successfully boots the Linux OS and runs various benchmarks, providing significant validation for the proposed method.}

\textbf{Weakness :} \textcolor{blue}{1. Limited Originality. While the paper extends existing methods, it lacks substantial innovation or originality in terms of Deep Learning methods. The application of Simulated Annealing to processor design seems well suited for other computer architecture conferences.}

Response 1: Our originality is to present an end-to-end machine learning based superscalar processor design flow, narrowing the performance gap between the automated design with state-of-the-art machine learning methods and human design. In this new application, the proposed method significantly outperforms the state-of-the-art automated processor design methods, and designs high-quality processors comparable with human designs without human involvement.

%第二段：我们方法的整个流程都是machine learning，首先将问题形式化为时序预测问题，是一个ml问题；然后我们具体的求解方法，包括模拟退火和BSD都是ml方法，整个过程都是ML的。

To achieve this goal, we propose an end-to-end machine learning methodology. First, we formalize the processor design task into a machine learning problem, i.e. the sequential prediction problem. We solve the problem with typical machine learning methods, i.e. the simulated annealing method and the BSD method. The key challenge of this specific ML problem is the high design accuracy in a large design space, so state-of-the-art methods including LLMs, NNs, Decision Trees, and BSDs can only design single-cycle processors with limited performance. We meet the challenge with a state selector learning to reduce the search space, and a state speculator to predict the specific sequence accurately. 

%第三段：我们还和做相同问题的ml方法进行了对比。他们做不好是因为xxx challenge，我们利用xxx ml方法解决了这个问题，性能提高xxx
We evaluate the proposed method with state-of-the-art machine learning methods. Compared with the state-of-the-art automated processor design methods, our method achieves a significant improvement of $382\times$ with the help of dependent data prediction. The design performance is comparable with ARM Cortex A53 CPUs in the 2010s, while no human efforts are involved in our end-to-end machine learning based design flow.


\textcolor{blue}{2. Clarity of Implementation Details. Some key implementation details and results are vaguely presented. The mechanism for recovering correct execution from incorrect value predictions is not clearly described, and it is unclear whether the results in Table 1 pertain to ASIC or FPGA implementations. Moreover, the explanations for the results shown in Figure 5, especially regarding predictions for PC and MEM, are not adequately clarified.}

Response 2: 

\textbf{(1) Error recovery.}

Also for Question: How do you ensure the accuracy of value predictions consistently? 

The dependent data predictor is formally verified to guarantee the on-the-fly predicting result is correct, i.e. the predictor only predicts the correct data and bypassed if there might be errors predicting the data.
In the experiment, we formally check the equivalence of the designed processor with the golden reference model, i.e. the single-cycle RISCV processor, in an SAT solver.
Suppose the data from the golden reference model is $Data_C$ and the designed processor is $Data_P$, there is a 1-bit signal $P$ showing whether the processor takes the predicted data. The checking formula is that $Data_C \neq Data_P \rightarrow P$
 
Let's see an example here, showing how the predicting accuracy can achieve 100\%. Given a branch instruction such as $if (a[31:0] > b[31:0]), pc=1000; else pc=8000$, it is difficult to predict the pc without actually execute the instruction with a 32-bit comparison. But in 25\% of the cases, a[31]=1 and b[31]=0, it is very easy to predict the branch and can be formally check with an SAT solver. Besides, the SAT solver is not on-the-fly in the processor, but a formal verification period while designing the predictor. When the predictor is $(a[31]==1 \&\& b[31]==0) \rightarrow pc=1000$, it is 
a formally correct predictor, although the predict coverage is only 25\%. Our ML method is trying to improve the predict coverage of the predictor, and all the covered predictions need to be formally accurate.

\textbf{(2) Evaluation settings.} 

The experiment is evaluated on ASIC design. We evaluate the result with a cycle-accurate simulator with Synopsys VCS. We run the standard CPU benchmark ARM Dhrystone multiple times in Synopsys VCS to evaluate the performance result. We verify the design functionality on Xilinx FPGA ZCU-104 and start Linux OS on the FPGA to make sure our design is correct. 
The hardware characteristics are ASIC with 45nm Technology according to the logic synthesis result in Synopsys Design Compiler. The FPGA is only used for verification, not to evaluate the hardware cost because our design is going to tapeout with an MPW shuttle this December.
 
 \textbf{(3)Results in Table 1.}
 
 {Also for Question: CPUs typically have caches, reducing the impact of memory access latency. Would the enhancements in your approach still be as significant if caches were incorporated?}

S-BSD improves the processor performance more than only caching. It predicts the intermediate results that can be reused in both the computational part and the memory part, while caching can only accelerate the memory process. In the paper, We compare the performance with human-designed cached CPUs in Section 5.2. 

Our evaluation focuses on comparing the design performance with the state-of-the-art automated design methods, to show how our method significantly narrows the gap between design by ML methods and design by human experts. Current automated processor designs with state-of-the-art methods cannot analyse the dependencies in the execution, so that the design has very limited performance than ours without caching or other throughput optimization techniques.

According to your question, We add another experiment to show our method contributes in both the computational part and memory part. With only an extra human-designed cache, the state-of-the-art automated designed CPU \textit{Enlightenment-1}'s throughput is 3985837 Dhrystone/s. The result shows that the memory part introduces 245.7 improvement and the computational part introduces 1.55x improvement comparing to the state-of-the-art automated design methods. Thanks for the insightful question, and the analysis will be added in the revision.


\textbf{Limitations:}
\textcolor{blue}{The authors adequately addressed the limitations and, if applicable, potential negative societal impact of their work.}

\textbf{Flag For Ethics Review:} \textcolor{blue}{No ethics review needed.}

\textbf{Rating:} \textcolor{blue}{5: Borderline accept: Technically solid paper where reasons to accept outweigh reasons to reject, e.g., limited evaluation. Please use sparingly.}

\textbf{Confidence:} \textcolor{blue}{3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.}

\textbf{Code Of Conduct:} \textcolor{blue}{Yes}


%第二段：加实验，分析结果
%In detail, We run an additional experiment with our design comparing the CPU with the same caching strategy. The result shows that compared with a baseline CPU with cache, the predictors for PC/GPR of the proposed method contribute to the overall result with xxx(about 20\%) improvement. In more detail, We evaluate the result with a cycle-accurate simulator with Synopsys VCS. In the experiment, the Verilog code is generated with S-BSD but only 1 predictor for MEM (comparing our proposed design with all 3 predictors). With clock period = 2GHz, the Dhrystone result of the cached-baseline CPU is xxx, while the result of our proposed CPU is xxx. These experimental results show that our method contributes to both memory and computation. This experiment will be added in the revision.

%第三段：强调我们是和自动化方法在比。（给现在的自动化方法一个cache，他也用不好）
 %It is challenging to design processors automatically with caches for state-of-the-art methods including LLMs, NNs, Decision Trees, and BSDs, because these methods cannot guarantee design correctness in such a large design space. We meet this challenge with the state selectors and state speculators. The proposed method correctly designs the superscalar processor for the first time, and it can run the Linux OS. In this way, our method achieves significant performance improvement compared with the state-of-the-art automated processor design.


%\textbf{In figure 2, the illustration could be improved. For instance, the dots in selector region could be aligned. The sub-figure in speculator region could be enlarged.}
%修改图，放在pdf里，传上去（看一下rebuttal改图的要求

%Thanks. It will be revised in the revision.




